Medical Reasoning with Large Language Models: A Survey and MR-Bench

Large language models (LLMs) have achieved strong performance on medical exam-style tasks, motivating growing interest in their deployment in real-world clinical settings. However, clinical decision-making is inherently safety-critical, context-dependent, and conducted under evolving evidence. In such situations, reliable LLM performance depends not on factual recall alone, but on robust medical reasoning. In this work, we present a comprehensive review of medical reasoning with LLMs. Grounded in cognitive theories of clinical reasoning, we conceptualize medical reasoning as an iterative process of abduction, deduction, and induction, and organize existing methods into seven major technical routes spanning training-based and training-free approaches. We further conduct a unified cross-benchmark evaluation of representative medical reasoning models under a consistent experimental setting, enabling a more systematic and comparable assessment of the empirical impact of existing methods. To better assess clinically grounded reasoning, we introduce MR-Bench, a benchmark derived from real-world hospital data. Evaluations on MR-Bench expose a pronounced gap between exam-level performance and accuracy on authentic clinical decision tasks. Overall, this survey provides a unified view of existing medical reasoning methods, benchmarks, and evaluation practices, and highlights key gaps between current model performance and the requirements of real-world clinical reasoning.

==> sections/intro_v0.tex <==
\section{Introduction}\label{section1}

Large language models (LLMs) are rapidly permeating biomedical and clinical workflows \cite{artsi2025large}, supporting Electronic Health Record (EHR) summarization \cite{croxford2025evaluating}, clinical documentation \cite{takayama2025evaluating}, patient communication \cite{busch2025current}, literature synthesis \cite{delgado2025transforming}, and clinical decision support \cite{oniani2024enhancing}. Early studies \cite{kung2023usmle,nori2023gpt4,moor2023foundation,singhal2023large} show that \textcolor{blue}{foundation language models such as GPT3.5 \cite{kung2023usmle} and Med-PALM \cite{singhal2023large}} reach passing performance on standardized medical examinations and can answer many knowledge-intensive medical questions, indicating substantial encoded biomedical and clinical knowledge. For effective clinical practice and deployment, which increasingly involves evaluating LLMs as clinical decision support co-pilots—providing diagnostic assistance in radiology and genomics, and serving as tools for medical education and training \cite{maity2025large,singhal2023large}—this static knowledge is essential to be continually updated with frontier research \cite{grol2003best}.

Given the high-stakes and low-error-tolerance nature of \textcolor{blue}{clinical environments \cite{xu2025artificial}, effective clinical decision-making by LLMs fundamentally hinges on medical reasoning \cite{bedi2025fidelity}} Medical reasoning is essential to prevent critical failures, such as fabricating details or miscalibrating uncertainty, which are unacceptable in clinical settings \cite{ji2023hallucination, kadavath2022know}. \textcolor{blue}{However, while prevalent medical QA benchmarks often serve as proxies to simulate this complex decision-making process, they substantially originate from standardized examinations rather than authentic clinical environments \cite{jin2021disease}.} \textcolor{blue}{Although recent gains on medical QA benchmarks are encouraging \cite{kung2023usmle, nori2023gpt4}, performance notably degrades when models are confronted with the complexities of real-world clinical environments, which demand multi‑step inference, causal understanding, and careful handling of ambiguity \cite{moor2023foundation}.} This gap raises a central question: do these systems perform genuine, reliable reasoning? We argue that verifiable medical reasoning is a necessary precondition for the safe and effective integration of LLMs into clinical practice.


Medical reasoning is a complex cognitive process involving iterative information gathering, hypothesis generation, and synthesis for clinical decision-making \cite{barrows1987clinical}. The hypothetico-deductive model \cite{edwards2004clinical} frames this cognitive workflow as an iterative process of abductive hypothesis generation, deductive testing, and inductive confirmation. Inspired by this, we categorize medical reasoning capabilities into three dimensions: medical abduction, the formulation of plausible differential diagnoses from initial clinical findings \cite{ward1997abductive}; medical deduction, the systematic testing of these candidate diagnoses to predict expected symptoms or select distinguishing diagnostic tests \cite{croskerry2009clinical}; and medical induction, the synthesis of accumulating evidence to determine the most probable diagnosis \cite{stanley2013logic}. Accordingly, to support these intertwined forms of medical reasoning, we posit that medical reasoning LLMs require: (1) a comprehensive and accurate medical knowledge base that serves as a solid foundation for subsequent analytical tasks, demanding a powerful base model \cite{li202512surveyreasoning}; (2) the capacity for active information acquisition to support iterative data gathering and context interpretation; and (3) structured, multi-step reasoning processes to drive hypothesis generation and conclusion synthesis, aligning with frontier reasoning models \cite{guo2025deepseekr1}.




\textcolor{blue}{While a recent survey has provided a preliminary summary of research paradigms for medical reasoning LLMs \cite{berger2025reasoning}, it lacks a deep, critical analysis of the current research landscape. Addressing this limitation,} this paper presents a structured review of the current state of reasoning LLMs in the medical domain. We begin by categorizing contemporary methodologies into two primary paradigms: training-based approaches, encompassing continued pretraining \cite{gururangan-etal-2020-dont}, supervised fine-tuning \cite{wei2022finetuned}, and reinforcement learning \cite{ouyang2022training}; and training-free approaches, which include prompt engineering \cite{liu2023pre}, test-time strategies \cite{wang2022self}, retrieval and tool use \cite{lewis2020rag}, agentic pipelines \cite{xi2025rise}. Following this review, we summarize prevalent benchmarks and evaluation methodologies and conduct a comprehensive evaluation of these approaches across multiple benchmarks.

Furthermore, we systematically analyze the critical limitations of prevailing benchmarks. To concretely demonstrate specific deficiencies in existing evaluation paradigms, we conduct detailed case studies on representative datasets, including \textbf{MedQA} \cite{jin2021disease} and \textbf{HealthBench} \cite{arora2025healthbench}. Our analysis points to potential limitations in representative benchmarks: widely used QA datasets like MedQA occasionally lack critical information required for reasoning, while open-ended frameworks like HealthBench—relying on the LLM-as-a-judge paradigm—can exhibit scoring sensitivity to evaluator variations. To better evaluate the medical reasoning capabilities of LLMs, we introduce \textbf{MR-Bench}, a novel benchmark derived entirely from real-world clinical data \cite{johnson2016mimic, johnson2023mimic}. 
%It encompasses two challenging, clinically relevant tasks including medication imputation, procedure selection.
It encompasses two challenging, clinically relevant tasks—\textit{medication imputation} and \textit{procedure selection}—in which models need to (i) complete partially masked inpatient medication orders and (ii) select the appropriate set of procedures for an admission based on the available clinical evidence.
Our experiments reveal a striking disparity: even advanced foundation models (e.g., GPT-5), which achieve near-perfect scores on standard medical licensing examinations, exhibit significant performance gaps on these authentic clinical tasks. These findings highlight that current LLMs remain distant from being truly "deployment-ready" for clinical practice. Consequently, MR-Bench offers a vital new perspective for evaluating medical reasoning, steering future research toward practical clinical utility.

==> sections/sec2_v0.tex <==
\section{Approaches for Medical Reasoning with LLMs}\label{section2}
To orient researchers to recent advances in utilizing LLMs for medical reasoning, this section surveys the principal technical routes for training and adapting LLMs (given space constraints, we do not provide additional discussion of multimodal LLM methods). Table~\ref{table 1} provides an overview of these routes and representative studies. We group methods into two families. Training-base approaches—continued pretraining (domain adaptation), supervised fine-tuning, and reinforcement learning—offer strong domain alignment but are compute-intensive and are preferable when resources permit. Training-free approaches—prompt engineering, test-time inference strategies, retrieval and tool use, agentic pipelines—keep the backbone frozen and are practical under constrained compute budgets. Together, these seven routes summarize current practice for building medical reasoning models.


\begin{table}[!htbp]
\centering
\caption[Approaches for Medical Reasoning with LLMs]{Approaches for Medical Reasoning with LLMs. \protect\underline{Underlined}: Open-source. \protect\colorbox{yellow!30}{Yellow}: Research focused on model training. \protect\colorbox{green!10}{Green}: Research utilizing LLMs as tools (e.g., agents).}
\label{table 1}
% Use tabularx to make the table the full text width
% 'l' = left-aligned
% 'X' = an auto-wrapping, flexible-width column
\begin{tabularx}{\textwidth}{p{2.6cm} p{3.4cm} >{\raggedright\arraybackslash}X}
\toprule
\textbf{Category} & \textbf{Approach} & \textbf{Research} \\
\midrule

% --- Weight-Update Section ---
\multirow{15}{=}{Training-based approaches} 
& Continue pretraining & \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M1}} \cite{wang2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M2}} \cite{dou2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{MedFound}} \cite{liu2025generalist}, \protect\colorbox{yellow!30}{\protect\underline{Citrus}} \cite{wang2025citrus}, \protect\colorbox{yellow!30}{\protect\underline{EHR-R1}} \cite{liao2025ehr} \\
\cmidrule(l){2-3} 
& Supervised fine-tuning & \protect\colorbox{yellow!30}{Med-PALM} \cite{singhal2023large}, \protect\colorbox{yellow!30}{Med-PALM 2} \cite{singhal2025toward}, \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M1}} \cite{wang2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M2}} \cite{dou2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{Lingshu}} \cite{xu2025lingshu}, \protect\colorbox{yellow!30}{\protect\underline{HuatuoGPT-o1}} \cite{chen2412huatuogpt}, \protect\colorbox{yellow!30}{\protect\underline{UltraMedical}} \cite{zhang2024ultramedical}, \protect\colorbox{yellow!30}{\protect\underline{m1}} \cite{huang2025m1}, \protect\colorbox{yellow!30}{\protect\underline{MedReason}} \cite{wu2025medreason}, \protect\colorbox{yellow!30}{\protect\underline{BioMed-R1}} \cite{thapa2025disentangling}, \protect\colorbox{yellow!30}{\protect\underline{MedS$^{3}$}} \cite{jiang2025meds}, \protect\colorbox{yellow!30}{\protect\underline{Med-Gemma}} \cite{sellergren2025medgemma}, \protect\colorbox{green!10}{\protect\underline{DrugGPT}} \cite{zhou2025collaborative}, \protect\colorbox{yellow!30}{\protect\underline{MedFound}} \cite{liu2025generalist}, \protect\colorbox{yellow!30}{Med-Gemini} \cite{saab2024capabilities}, \protect\colorbox{yellow!30}{\protect\underline{LongMonolog}} \cite{huang2025o1}, \protect\colorbox{green!10}{\protect\underline{MedResearcher-R1}} \cite{yu2025medresearcher}, \protect\colorbox{yellow!30}{\protect\underline{Citrus}} \cite{wang2025citrus}, \protect\colorbox{yellow!30}{\protect\underline{ClinicalGPT-R1}} \cite{lan2025clinicalgpt}, \protect\colorbox{yellow!30}{AMIE} \cite{mcduff2025towards, tu2025towards}, \protect\colorbox{green!10}{\protect\underline{MedAgentGym}} \cite{xu2025medagentgym}, \protect\colorbox{green!10}{\protect\underline{DiagnoseGPT}} \cite{chen2025cod}, \protect\colorbox{green!10}{\protect\underline{DDO}} \cite{jia2025ddo}, \protect\colorbox{yellow!30}{\protect\underline{Meerkat}} \cite{kim2025small}, \protect\colorbox{green!10}{\protect\underline{Self-BioRAG}} \cite{jeong2024improving}, \protect\colorbox{yellow!30}{\protect\underline{Med42-v2}} \cite{christophe2024med42v2}, \protect\colorbox{green!10}{\protect\underline{MedAdapter}} \cite{shi2024medadapter}, \protect\colorbox{yellow!30}{QuarkMed} \cite{li2025quarkmed}, \protect\colorbox{yellow!30}{\protect\underline{EHR-R1}} \cite{liao2025ehr} \\
\cmidrule(l){2-3}
& Reinforcement learning & \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M1}} \cite{wang2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{Baichuan-M2}} \cite{dou2025baichuan}, \protect\colorbox{yellow!30}{\protect\underline{Lingshu}} \cite{xu2025lingshu}, \protect\colorbox{yellow!30}{\protect\underline{HuatuoGPT-o1}} \cite{chen2412huatuogpt}, \protect\colorbox{yellow!30}{\protect\underline{UltraMedical}} \cite{zhang2024ultramedical}, \protect\colorbox{yellow!30}{\protect\underline{m1}} \cite{huang2025m1}, \protect\colorbox{yellow!30}{\protect\underline{BioMed-R1}} \cite{thapa2025disentangling}, \protect\colorbox{yellow!30}{\protect\underline{AlphaMed}} \cite{liu2025beyond}, \protect\colorbox{yellow!30}{\protect\underline{MedS$^{3}$}} \cite{jiang2025meds}, \protect\colorbox{yellow!30}{\protect\underline{Med-Gemma}} \cite{sellergren2025medgemma}, \protect\colorbox{yellow!30}{\protect\underline{MedFound}} \cite{liu2025generalist}, \protect\colorbox{yellow!30}{\protect\underline{MedResearcher-R1} }\cite{yu2025medresearcher}, \protect\colorbox{yellow!30}{\protect\underline{Citrus}} \cite{wang2025citrus}, \protect\colorbox{yellow!30}{\protect\underline{ClinicalGPT-R1}} \cite{lan2025clinicalgpt}, \protect\colorbox{green!10}{\protect\underline{DDO}} \cite{jia2025ddo}, \protect\colorbox{green!10}{\protect\underline{Deep-DxSearch}} \cite{zheng2025end}, \protect\colorbox{yellow!30}{\protect\underline{AdaThink-Med}} \cite{rui2025adathink}, \protect\colorbox{yellow!30}{\protect\underline{Med42-v2}} \cite{christophe2024med42v2}, \protect\colorbox{yellow!30}{QuarkMed} \cite{li2025quarkmed}, \protect\colorbox{yellow!30}{\protect\underline{EHR-R1}} \cite{liao2025ehr} \\

\midrule 

% --- No-Weight-Update Section ---
\multirow{18}{=}{Training-free approaches} 
& Prompt engineering & \protect\colorbox{yellow!30}{Med-PALM} \cite{singhal2023large}, \protect\colorbox{yellow!30}{Med-PALM 2} \cite{singhal2025toward}, \protect\colorbox{yellow!30}{\protect\underline{HuatuoGPT-o1}} \cite{chen2412huatuogpt}, \protect\colorbox{yellow!30}{\protect\underline{UltraMedical}} \cite{zhang2024ultramedical}, \protect\colorbox{yellow!30}{\protect\underline{m1}} \cite{huang2025m1}, \protect\colorbox{yellow!30}{\protect\underline{MedReason}} \cite{wu2025medreason}, \protect\colorbox{yellow!30}{\protect\underline{BioMed-R1}} \cite{thapa2025disentangling}, \protect\colorbox{yellow!30}{\protect\underline{MedS$^{3}$}} \cite{jiang2025meds}, \protect\colorbox{yellow!30}{\protect\underline{Med-Gemma}} \cite{sellergren2025medgemma}, \protect\colorbox{green!10}{\protect\underline{DrugGPT}} \cite{zhou2025collaborative}, \protect\colorbox{yellow!30}{\protect\underline{MedFound}} \cite{liu2025generalist}, \protect\colorbox{yellow!30}{Med-Gemini} \cite{saab2024capabilities}, \protect\colorbox{green!10}{\protect\underline{CLINICR}} \cite{sandeep2024few}, \protect\colorbox{green!10}{EnsReas} \cite{lucas2024reasoning}, \protect\colorbox{yellow!30}{AMIE} \cite{mcduff2025towards, tu2025towards}, \protect\colorbox{green!10}{\protect\underline{Medprompt}} \cite{nori2023can}, \protect\colorbox{green!10}{\protect\underline{Clinical CoT}} \cite{kwon2024large}, \protect\colorbox{green!10}{DR-CoT} \cite{wu2023large}, \protect\colorbox{green!10}{Diagnostic reasoning prompts} \cite{savage2024diagnostic}, \protect\colorbox{green!10}{\protect\underline{DiagnoseGPT}} \cite{chen2025cod}, \protect\colorbox{green!10}{\protect\underline{MEDIQ}} \cite{li2024mediq}, \protect\colorbox{yellow!30}{\protect\underline{Meerkat}} \cite{kim2025small}, \protect\colorbox{green!10}{\protect\underline{MedRAG}} \cite{zhao2025medrag}, \protect\colorbox{green!10}{\protect\underline{MedAdapter}} \cite{shi2024medadapter} \\
\cmidrule(l){2-3}
& Test-time strategies & \protect\colorbox{yellow!30}{Med-PALM} \cite{singhal2023large}, \protect\colorbox{yellow!30}{Med-PALM 2} \cite{singhal2025toward}, \protect\colorbox{yellow!30}{\protect\underline{m1}} \cite{huang2025m1}, \protect\colorbox{yellow!30}{\protect\underline{LongMonolog}} \cite{huang2025o1}, \protect\colorbox{yellow!30}{Med-Gemini} \cite{saab2024capabilities}, \protect\colorbox{green!10}{\protect\underline{CLINICR}} \cite{sandeep2024few}, \protect\colorbox{green!10}{EnsReas} \cite{lucas2024reasoning}, \protect\colorbox{green!10}{\protect\underline{Medprompt}} \cite{nori2023can}, \protect\colorbox{green!10}{\protect\underline{MEDIQ}} \cite{li2024mediq}, \protect\colorbox{yellow!30}{\protect\underline{Meerkat}} \cite{kim2025small}, \protect\colorbox{green!10}{\protect\underline{MedAdapter}} \cite{shi2024medadapter} \\
\cmidrule(l){2-3}
& Retrieval and tool use & \protect\colorbox{yellow!30}{Med-PALM 2} \cite{singhal2025toward}, \protect\colorbox{green!10}{\protect\underline{DrugGPT}} \cite{zhou2025collaborative}, \protect\colorbox{yellow!30}{Med-Gemini} \cite{saab2024capabilities}, \protect\colorbox{green!10}{\protect\underline{MedRaC}} \cite{medrac2024from}, \protect\colorbox{green!10}{\protect\underline{MedResearcher-R1}} \cite{yu2025medresearcher}, \protect\colorbox{green!10}{\protect\underline{Medprompt}} \cite{nori2023can}, \protect\colorbox{green!10}{\protect\underline{DiagnoseGPT}} \cite{chen2025cod}, \protect\colorbox{green!10}{\protect\underline{Deep-DxSearch}} \cite{zheng2025end}, \protect\colorbox{green!10}{\protect\underline{MedRAG}} \cite{zhao2025medrag}, \protect\colorbox{green!10}{\protect\underline{Self-BioRAG}} \cite{jeong2024improving}, \protect\colorbox{yellow!30}{QuarkMed} \cite{li2025quarkmed} \\
\cmidrule(l){2-3}
& Agentic pipelines & \protect\colorbox{green!10}{\protect\underline{DrugGPT}} \cite{zhou2025collaborative}, \protect\colorbox{yellow!30}{AMIE} \cite{mcduff2025towards, tu2025towards}, \protect\colorbox{green!10}{\protect\underline{MedAgents}} \cite{tang2024medagents}, \protect\colorbox{green!10}{\protect\underline{MedAgentGym}} \cite{xu2025medagentgym}, \protect\colorbox{green!10}{\protect\underline{DiagnoseGPT}} \cite{chen2025cod}, \protect\colorbox{green!10}{\protect\underline{MEDIQ}} \cite{li2024mediq}, \protect\colorbox{green!10}{\protect\underline{DDO}} \cite{jia2025ddo}, \protect\colorbox{green!10}{\protect\underline{Deep-DxSearch}} \cite{zheng2025end}, \protect\colorbox{green!10}{\protect\underline{MedRAG}} \cite{zhao2025medrag}, % 在 Agentic pipelines 这一行的末尾添加：
\protect\colorbox{green!10}{\protect\underline{MedChain-Agent}} \cite{liu2025medchain}, \protect\colorbox{green!10}{PHA} \cite{heydari2025anatomy} \\


\bottomrule
\end{tabularx}


% --------------------------------
\end{table}




\subsection{Training-Based Approaches}

\noindent \textbf{Continued Pretraining.}
LLM pretraining constitutes the initial training phase, wherein a model is exposed to a massive corpus of unlabeled text using a self-supervised objective, such as next-token prediction, to acquire foundational linguistic capabilities and broad world knowledge \cite{brown2020language}. Continued pretraining, also termed domain-adaptive pretraining, builds upon a foundational general model by further training it on a curated corpus specific to a target domain, such as medicine \cite{gu2021domain}. The primary objective is twofold: to deeply embed specialized medical knowledge for enhanced pattern recognition and factual recall \cite{wang2025citrus}, and to establish a reliable knowledge foundation for a model's subsequent, deliberate analytical reasoning processes \cite{wei2022chain, marwala2024thinking, bellini2024dual}.

Methodologies for this adaptation vary. Some efforts, such as the development of MedFound \cite{liu2025generalist, workshop2022bloom}, prioritize scale and diversity by pretraining on massive corpora that amalgamate medical literature with real-world clinical data. Other strategies, like that for Baichuan-M1 \cite{wang2025baichuan}, employ a more curated, staged curriculum that progressively introduces more complex medical data. A distinct approach, exemplified by Baichuan-M2 \cite{dou2025baichuan}, involves augmenting the pretraining corpus itself, for instance, by systematically injecting explicit reasoning traces or logical structures to directly expose the model to transferable reasoning patterns. In the context of EHRs, EHR-R1 \cite{liao2025ehr} performs large-scale domain adaptation on 3.5 million structured patient records to align the model with longitudinal clinical distributions. Collectively, these studies establish continued pretraining as a vital step to ground LLMs in the medical domain, creating a knowledge-rich foundation for subsequent fine-tuning.





\noindent \textbf{Supervised Fine-Tuning.}
Supervised Fine-Tuning (SFT), often referred to as instruction tuning, adapts pre-trained models to specific tasks using high-quality input-output examples \cite{ouyang2022training}. In medical reasoning, SFT is one of the primary mechanisms for instilling deliberate analytical capabilities \cite{huang-chang-2023-towards}. Training on exemplars with explicit reasoning steps, such as Chain-of-Thought (CoT), aligns the model to produce structured, step-by-step analyses instead of just direct answers \cite{wei2022chain}.

The quality and nature of the SFT dataset are critical. The gold standard is data meticulously crafted by human experts (e.g., Med-PALM \cite{singhal2023large}/Med-PALM 2 \cite{singhal2025toward}, AMIE \cite{mcduff2025towards, tu2025towards}). Due to the high cost, many studies employ bootstrapping, where a model generates its own training data. This ranges from self-bootstrapping from seeds (MedFound \cite{liu2025generalist}) to algorithmic exploration of reasoning paths (MedS$^3$ \cite{jiang2025meds}). A more common approach is knowledge distillation, distilling a "teacher" model's (e.g., GPT-4o, Deepseek R1 etc.) capabilities into a "student" \cite{kwon2024large}. This includes complex methods where teachers verify reasoning trajectories (e.g., HuatuoGPT-o1 \cite{chen2412huatuogpt}, ClinicalGPT-R1 \cite{lan2025clinicalgpt}) or even synthesizing reasoning chains directly from raw medical textbooks to ensure high-quality, hallucination-free guidance, as seen in Meerkat \cite{kim2025small}. Similarly, EHR-R1 \cite{liao2025ehr} utilizes a ``thinking-graph'' pipeline to synthesize 300k reasoning-rich instances by grounding extracted EHR entities in medical knowledge graphs. Notably, DiagnoseGPT \cite{chen2025cod} utilizes the Chain of Diagnosis (CoD) framework to structure SFT around clinical logic—spanning symptom abstraction to disease recall—thereby enhancing diagnostic interpretability. Self-BioRAG \cite{jeong2024improving} takes this further by employing a "critic" model to annotate instruction data with reflective tokens (e.g., assessing relevance or support), allowing the generator to learn self-assessment behaviors during fine-tuning. Datasets are also often enriched with external knowledge graph or tools (e.g., MedReason \cite{wu2025medreason}, Med-Gemini \cite{saab2024capabilities}).

Finally, SFT is frequently the initial "cold start" stage in multi-stage paradigms, most notably SFT followed by Reinforcement Learning (RL). SFT provides foundational reasoning policies and output alignment, which RL then refines. This dominant SFT+RL approach is employed by models like Baichuan-M1/M2 \cite{wang2025baichuan, dou2025baichuan}, Citrus \cite{wang2025citrus}, Lingshu \cite{xu2025lingshu}, and Med-Gemma \cite{sellergren2025medgemma, gemmateam2025gemma3technicalreport}. The paradigm also extends to training complex agentic systems (e.g., MedAgentGym \cite{xu2025medagentgym}, DDO \cite{jia2025ddo}).




\noindent \textbf{Reinforcement Learning.}
The feasibility of using RL to enhance LLM reasoning was highlighted by DeepSeek-R1 \cite{guo2025deepseekr1}.RL optimizes model policies via feedback, aiming for more accurate or reliable outcomes beyond simple imitation \cite{ouyang2022training}. This process enhances the robustness of deliberate analytical capabilities. While often used to refine policies initialized during SFT, RL implementations generally follow two main paradigms: policy-gradient methods using an explicit reward model, and preference-based methods learning from comparisons.

The first paradigm employs policy-gradient algorithms, like Proximal Policy Optimization (PPO) \cite{schulman2017proximal}, guided by an RM that scores the quality of generated reasoning. This approach is used by HuatuoGPT-o1 \cite{chen2412huatuogpt}, ClinicalGPT-R1 \cite{lan2025clinicalgpt}, and the DDO agent \cite{jia2025ddo}. More advanced variants, such as Group Relative Policy Optimization (GRPO) \cite{shao2024deepseekmath}, are used for stable training by Lingshu \cite{xu2025lingshu}, Baichuan-M2 \cite{dou2025baichuan}, BioMed-R1 \cite{thapa2025disentangling}, EHR-R1 \cite{liao2025ehr}, and MedResearcher-R1 \cite{yu2025medresearcher}. AlphaMed \cite{liu2025beyond} also employs GRPO but uniquely demonstrates that reasoning can emerge purely through rule-based RL on multiple-choice questions without relying on distilled CoT supervision or complex reward models. The design of the reward function is therefore critical, ranging from simple binary rewards (AlphaMed \cite{liu2025beyond}) to hybrid rule/model-based reward models (Baichuan-M1 \cite{wang2025baichuan}, Baichuan-M2 \cite{dou2025baichuan}) and complex multi-dimensional evaluations (Deep-DxSearch \cite{zheng2025end}).

Alternatively, preference-based methods like Direct Preference Optimization (DPO) \cite{rafailov2023direct} learn directly from preference pairs (i.e., 'chosen' vs. 'rejected') without an explicit reward model. DPO is used by MedFound \cite{liu2025generalist} to align with expert preferences, by MedS$^{3}$ \cite{jiang2025meds} to refine trajectories from Monte Carlo Tree Search (MCTS), and by UltraMedical \cite{zhang2024ultramedical} in an iterative loop in an iterative loop that explores DPO and Kahneman-Tversky Optimization (KTO) \cite{ethayarajh2024kto}. Other offline RL methods are also employed, such as in Citrus \cite{wang2025citrus}, which adopts Contrastive Preference Optimization (CPO) and Simple Preference Optimization (SimPO) \cite{meng2024simpo}, and Med-Gemma \cite{sellergren2025medgemma}, to sharpen the model's analytical acuity post-SFT.

\subsection{Training-Free Approaches}

\noindent \textbf{Prompt Engineering.}
Prompt engineering refers to carefully crafting input prompts to obtain specific and controlled responses from LLMs \cite{liu2023pre}. The foundational technique in this category is CoT prompting, which elicits reasoning by instructing the model to generate intermediate, step-by-step analytical steps before providing a final answer \cite{wei2022chain}. Several foundational medical models, including the Med-PALM series \cite{singhal2023large, singhal2025toward} and AMIE \cite{mcduff2025towards, tu2025towards}, rely on CoT prompting to elicit diagnostic reasoning.

Beyond basic CoT, a significant line of inquiry involves tailoring prompts to specifically mimic clinical cognitive workflows. This moves beyond generic "step-by-step" instructions; for example, Clinical CoT \cite{kwon2024large}, DR-CoT (Diagnostic-Reasoning CoT) \cite{wu2023large}, and Diagnostic Reasoning Prompts \cite{savage2024diagnostic} explicitly frame the reasoning process as a formal differential diagnosis, while CLINICR \cite{sandeep2024few} simulates the incremental information-gathering process. MedRAG \cite{zhao2025medrag} utilizes a specific "KG-elicited reasoning" prompt that forces the model to explicitly consider the diagnostic differences retrieved from a constructed knowledge graph. Other advanced strategies optimize the prompt's examples or embed it in an agentic framework. Medprompt \cite{nori2023can}, for instance, uses k-NN to dynamically retrieve the most relevant few-shot examples for each new question. Meanwhile, DiagnoseGPT \cite{chen2025cod} designs a structured, five-step prompting pipeline, and MEDIQ \cite{li2024mediq} uses an interactive framework that allows the model to decide whether to answer or ask clarifying questions.

Finally, prompt engineering plays a crucial dual role, serving not only as an inference-time strategy but also as a critical component for generating SFT training data. Models like HuatuoGPT-o1 \cite{chen2412huatuogpt}, UltraMedical \cite{zhang2024ultramedical}, m1 \cite{huang2025m1}, and MedReason \cite{wu2025medreason} all use sophisticated prompting of teacher models to create high-quality, reasoning-rich exemplars. This technique is also integral to the data-generation pipelines for models such as BioMed-R1 \cite{thapa2025disentangling}, MedS$^{3}$ \cite{jiang2025meds}, Med-Gemma \cite{sellergren2025medgemma}, DrugGPT \cite{zhou2025collaborative}, MedFound \cite{liu2025generalist}, Med-Gemini \cite{saab2024capabilities}, and Meerkat \cite{kim2025small}.

\noindent \textbf{Test-Time Strategies.}
Test-time strategies enhance reasoning at the point of inference by manipulating the decoding process, often involving ensembles or iterative refinement to improve robustness over a single greedy output. The most foundational approach is Self-Consistency (SC), which samples multiple diverse reasoning paths and selects the final answer via a majority vote \cite{wang2022self}. This technique was notably employed by Med-PALM \cite{singhal2023large}, Med-PALM 2 \cite{singhal2025toward}, and as an option in MEDIQ \cite{li2024mediq}. Medprompt \cite{nori2023can} implements a specific variation for multiple-choice questions, using a "choice shuffling ensemble" that re-runs the prompt with permuted answer options to mitigate position bias before voting, a technique also adopted by Meerkat \cite{kim2025small}.

A more sophisticated line of inquiry uses iterative refinement, where the model's initial outputs are fed back into the system for critique or improvement. For example, Ensemble Refinement (ER) in Med-PALM 2 \cite{singhal2025toward} generates multiple answers and then prompts the model to synthesize them into a single, improved response. EnsReas \cite{lucas2024reasoning} adopts a more critical stance, re-prompting the model with its own conflicting reasoning paths to force a critical re-evaluation. Similarly, the "Forward-Backward" method of CLINICR \cite{sandeep2024few} first generates candidate diagnoses and then uses a verifier to select the most plausible one.

A final category involves dynamically allocating computational resources at inference. The "test-time scaling" or "inference-time scaling" approach, discussed in m1 \cite{huang2025m1} and LongMonolog \cite{huang2025o1}, operates on the principle that allowing a model a larger "thinking budget" (i.e., generating more tokens) improves accuracy on complex problems. Med-Gemini \cite{saab2024capabilities} presents an advanced form of this with its "uncertainty-guided search," an iterative loop that assesses the model's own confidence (via entropy) and dynamically triggers web searches to resolve uncertainty before finalizing an answer.


\noindent \textbf{Retrieval and Tool Use.}
To mitigate factual hallucinations and overcome the static knowledge limitations of LLMs, several approaches integrate external information at inference time. This paradigm, often called Retrieval-Augmented Generation (RAG) \cite{lewis2020rag}, grounds the model's reasoning in verifiable, domain-specific data, which is critical for high-stakes medical applications. These methods range from general-purpose web search, such as the "Chain of Retrieval" used by Med-PALM 2 \cite{singhal2025toward}, to queries against specialized, curated knowledge bases. For instance, DrugGPT \cite{zhou2025collaborative} queries structured drug and publication databases, while DiagnoseGPT \cite{chen2025cod} employs a retriever to recall candidate diseases from a dedicated database.

More sophisticated systems enhance this process. Med-Gemini \cite{saab2024capabilities} introduces an "uncertainty-guided search," an iterative loop that dynamically triggers web searches only when the model's internal confidence is low. Self-BioRAG \cite{jeong2024improving} internalizes this decision-making by training the model to generate specific tokens that trigger retrieval only when necessary. Other frameworks deploy a full suite of specialized tools. MedResearcher-R1 \cite{yu2025medresearcher} and Deep-DxSearch \cite{zheng2025end} utilize multiple, distinct retrievers to query clinical guidelines, match similar patient cases, and search PubMed, integrating these diverse information streams. MedRAG \cite{zhao2025medrag} constructs a hierarchical diagnostic knowledge graph to identify subtle distinctions between diseases with similar symptoms, injecting these "diagnostic differences" into the context alongside retrieved EHRs to improve diagnostic specificity.

Beyond factual retrieval, tools can offload specialized tasks that LLMs perform poorly, such as precise arithmetic. MedRaC \cite{medrac2024from}, for example, exemplifies this by first retrieving a medical formula and then invoking a Python code interpreter to perform the exact calculation, separating the task of reasoning from that of arithmetic. In a hybrid approach, retrieval can also be used to optimize the prompt itself. Medprompt \cite{nori2023can} uses k-NN retrieval not for factual grounding, but to dynamically select the most semantically relevant few-shot exemplars from a training set to construct the prompt for each new query.

\noindent \textbf{Agentic Pipelines.}
Agentic pipelines orchestrate reasoning, tool use, and planning into a cohesive framework to autonomously solve complex, multi-step problems \cite{wang2024survey}. Instead of a single response, an agent can execute a sequence of actions, observe outcomes, and adapt its plan, closely mimicking a cognitive workflow. In medicine, these pipelines are often designed to model the full diagnostic process.

One line of inquiry focuses on decomposing the task into a structured, pre-defined plan. For instance, the inference strategy for AMIE \cite{tu2025towards} follows a three-step sequence of analyzing information, formulating a response, and optimizing the output. DiagnoseGPT \cite{chen2025cod} implements a similar concept as a fixed five-step pipeline of symptom abstraction, disease recall, reasoning, confidence assessment, and decision-making. Other agents are designed for dynamic interaction; MEDIQ \cite{li2024mediq}, for example, operates within a framework where it must iteratively decide whether to make a final diagnosis or ask clarifying questions to gather more data. MedRAG \cite{zhao2025medrag} also incorporates an agentic component capable of identifying missing high-discriminability features in the knowledge graph to proactively generate follow-up questions.

Another prominent approach is multi-agent collaboration, where specialized roles are assigned to different LLM instances. MedAgents \cite{tang2024medagents} exemplifies this as a training-free framework where "expert" agents convene to analyze, discuss, and vote on a clinical case. DrugGPT \cite{zhou2025collaborative} also uses a multi-agent system, decomposing the task among an inquiry analysis agent, a knowledge acquisition agent, and an evidence generation agent.

Finally, complex systems involve explicitly training the agents, blurring the line between no-weight-update inference and a weight-updated model. AMIE \cite{mcduff2025towards, tu2025towards} uses an agentic "self-play" environment to generate high-quality SFT data. MedAgentGym \cite{xu2025medagentgym} provides a scalable environment specifically for training agents on code-centric biomedical data science tasks. This training often uses RL, as seen in DDO \cite{jia2025ddo}, which optimizes separate agents for inquiry and diagnosis, and Deep-DxSearch \cite{zheng2025end}, which trains an agent to jointly optimize its retrieval and reasoning policies.

==> sections/sec3_benchmarks_v0.tex <==
\section{Benchmarks and Evaluation - xh}\label{section3}

\subsection{Existing Benchmarks}
To evaluate the medical reasoning capabilities of LLMs, the research community has developed a series of benchmarks. As summarized in Table~\ref{Table 2}, these benchmarks primarily fall into two categories: medical-specific benchmarks and general-domain benchmarks whose medical subsets are commonly used for evaluation.



\begin{table}[htbp]
    \centering
    \caption{Summary of Existing Benchmarks. \protect\underline{Underlined} benchmarks represent general-domain datasets containing specific medical subsets.}
    \label{Table 2}
    \renewcommand{\arraystretch}{1.2} % 增加行高
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llc r}
        \toprule
        \textbf{Benchmark} & \textbf{Type} & \textbf{Year} & \textbf{Samples} \\
        \midrule
        % --- Multiple Choice QA ---
        \href{https://huggingface.co/datasets/qiaojin/PubMedQA}{PubMedQA} \cite{jin2019pubmedqa} & Multiple Choice QA & 2019 & 1,000 \\
        \href{https://huggingface.co/datasets/bigbio/med_qa}{MedQA (USMLE)} \cite{jin2021disease} & Multiple Choice QA & 2020 & 1,273 \\
        \href{https://huggingface.co/datasets/cais/mmlu}{\protect\underline{MMLU}} \cite{hendrycks2021measuring} & Multiple Choice QA & 2020 & 15,908 \\
        \href{https://huggingface.co/datasets/openlifescienceai/medmcqa}{MedMCQA (Validation)} \cite{pal2022medmcqa} & Multiple Choice QA & 2022 & 4,183 \\
        \href{https://huggingface.co/datasets/FreedomIntelligence/CMB}{CMBExam} \cite{wang2024cmb} & Multiple Choice QA & 2023 & 11,200 \\
        \href{https://huggingface.co/datasets/Idavidrein/gpqa}{\protect\underline{GPQA}} \cite{rein2024gpqa} & Multiple Choice QA & 2023 & 448 \\
        \href{https://huggingface.co/datasets/TIGER-Lab/MMLU-Pro}{\protect\underline{MMLU-Pro}} \cite{mmlu-pro} & Multiple Choice QA & 2024 & 12,032 \\
        \href{https://huggingface.co/datasets/mkieffer/Medbullets}{MedBullets} \cite{chen2025benchmarking} & Multiple Choice QA & 2024 & 308 \\
        \href{https://huggingface.co/datasets/guan-wang/ReDis-QA}{ReDis-QA} \cite{wang2024assessing} & Multiple Choice QA & 2024 & 1,360 \\
        \href{https://huggingface.co/datasets/cais/hle}{\protect\underline{HLE}} \cite{phan2025humanity} & Multiple Choice QA & 2025 & 2,500 \\
        \href{https://huggingface.co/datasets/jdh-algo/JMED}{JMED} \cite{wang2025citrus} & Multiple Choice QA & 2025 & 1,000 \\
        \href{https://huggingface.co/datasets/TsinghuaC3I/MedXpertQA}{MedXpertQA (Text)} \cite{zuo2025medxpertqa} & Multiple Choice QA & 2025 & 2,450 \\
        \href{https://huggingface.co/datasets/super-dainiu/medagents-benchmark}{MedAgentsBench} \cite{anonymous2025medagentsarena} & Multiple Choice QA & 2025 & 862 \\
        
        % --- Multiple Choice / Open Ended QA ---
        \href{https://huggingface.co/datasets/HPAI-BSC/CareQA}{Care-QA} \cite{Care-QA} & Multiple Choice / Open Ended QA & 2024 & 8,390 \\
        \href{https://github.com/ji-youn-kim/ehrnoteqa}{EHRNoteQA} \cite{kweon2024ehrnoteqa} & Multiple Choice / Open Ended QA & 2024 & 962 \\
        
        % --- Open Ended QA ---
        \href{https://huggingface.co/datasets/truehealth/medicationqa}{MedicationQA} \cite{singhal2023large} & Open Ended QA & 2022 & 690 \\
        \href{https://github.com/openai/simple-evals}{HealthBench} \cite{arora2025healthbench} & Open Ended QA & 2025 & 5,000 \\
        
        \href{https://huggingface.co/datasets/AIM-Harvard/MedBrowseComp}{MedBrowseComp} \cite{chen2025medbrowsecomp} & Open Ended QA & 2025 & 605 \\
        
        \href{https://github.com/MAGIC-AI4Med/MedRBench}{MedR-Bench} \cite{qiu2025quantifying} & Open Ended QA & 2025 & 1453 \\

        \href{https://ehrshot.stanford.edu/}{EHRSHOT} \cite{wornow2023ehrshot} & Clinical Risk Prediction & 2023 & 6,739 \\
        
        \href{https://github.com/paulhager/MIMIC-Clinical-Decision-Making-Dataset}{MIMIC-CDM} \cite{hager2024evaluation} & Clinical Decision Making & 2024 & 2,400 \\
        
        \href{https://github.com/MAGIC-AI4Med/EHR-R1}{EHR-Bench} \cite{liao2025ehr} & Clinical Decision Making / Risk Prediction & 2025 & 21,000 \\
        % --- Numerical Calculation ---
        \href{https://huggingface.co/datasets/ncbi/MedCalc-Bench-v1.0}{MedCalc-Bench} \cite{khandekar2024medcalc} & Numerical Calculation & 2024 & 1,047 \\

        \href{https://arxiv.org/abs/2508.20148}{PHA-Bench} \cite{heydari2025anatomy} & Personal Health Management & 2025 & 7,000+ \tnote{*}  \\
        \bottomrule
    \end{tabular*}

\end{table}

\noindent \textbf{Medical-Specific Benchmarks.}
The foundational layer of this category consists of datasets derived from standardized licensure examinations, serving as proxies for broad professional competency. Key examples include MedQA, derived from the United States Medical Licensing Examination (USMLE) \cite{jin2021disease}, MedMCQA \cite{pal2022medmcqa}, and CMBExam \cite{wang2024cmb}, which source multiple-choice questions (MCQs) from established medical entrance exams in the US, India, and China, respectively. Recent efforts have introduced benchmarks to address specific limitations of these standard exams. To test specialist-level reasoning and higher difficulty, MedBullets \cite{chen2025benchmarking} and MedXpertQA \cite{zuo2025medxpertqa} utilize questions in the style of advanced board exams (e.g., USMLE Step 2/3). To better simulate real-world clinical environments and ambiguity, JMED \cite{wang2025citrus} incorporates authentic case distributions and expanded option sets to mitigate random guessing, while Care-QA \cite{Care-QA} introduces open-ended assessment tasks. Furthermore, ReDis-QA \cite{wang2024assessing} specifically targets the complex reasoning required for rare disease diagnosis.

Beyond theoretical knowledge, a growing subset of benchmarks evaluates practical clinical utility and agentic capabilities. For information retrieval and evidence synthesis, PubMedQA \cite{jin2019pubmedqa} tests reasoning over biomedical literature, while MedBrowseComp \cite{chen2025medbrowsecomp} specifically assesses an agent's ability to browse, retrieve, and compare information across heterogeneous web sources. In the realm of patient interaction and clinical workflow, MedicationQA \cite{singhal2023large} and HealthBench \cite{arora2025healthbench} evaluate the quality and safety of responses to open-ended consumer health inquiries and multi-turn clinical conversations. Addressing specific functional deficits in LLMs, MedCalc-Bench \cite{khandekar2024medcalc} focuses on numerical accuracy in medical calculations, while EHRNoteQA \cite{kweon2024ehrnoteqa} evaluates the extraction and synthesis of information from electronic health records. 
Moving beyond extraction, EHRSHOT \cite{wornow2023ehrshot} focuses on longitudinal clinical risk prediction. MIMIC-CDM \cite{hager2024evaluation} further advances evaluation into interactive settings requiring active information gathering, while EHR-Bench \cite{liao2025ehr} consolidates these challenges into a comprehensive suite spanning 42 distinct decision-making and risk prediction tasks. To address the complexity of personal health management, PHA-Bench \cite{heydari2025anatomy} leverages the WEAR-ME dataset to evaluate agents across 10 diverse tasks spanning data science analysis, clinical reasoning, and health coaching, utilizing over 7,000 human annotations. Furthermore, MedAgentsBench \cite{anonymous2025medagentsarena} is tailored to evaluate multi-agent collaboration in solving complex medical problems. Complementing these, MedR-Bench \cite{qiu2025quantifying} utilizes 1,453 structured patient cases derived from PMC Open Access case reports to systematically evaluate LLMs across three critical stages of clinical care: examination recommendation, diagnostic decision-making, and treatment planning. Moreover, MedChain \cite{liu2025medchain} introduces a sequential benchmark of 12,163 cases that enforces a strict five-stage clinical workflow. Uniquely, it utilizes a ``Patient Agent'' to simulate real-time doctor-patient dialogue, requiring models to actively gather scattered information through conversation rather than processing static context.

\noindent \textbf{General-Domain Benchmarks.}
While specialized medical benchmarks test domain knowledge, general-purpose benchmarks with distinct medical subsets are increasingly used to evaluate the underlying reasoning engines of LLMs \cite{nori2023can, singhal2023large}. These benchmarks often feature higher abstraction levels and are less susceptible to contamination from medical training corpora \cite{rein2024gpqa, phan2025humanity}. MMLU \cite{hendrycks2021measuring} remains the de facto standard, with its six clinical and biological subtasks (e.g., Professional Medicine, Anatomy) serving as a primary barometer for general medical intelligence. Its successor, MMLU-Pro \cite{mmlu-pro}, introduces harder reasoning requirements and a larger option space (10 options) to provide a more robust signal of capability. For assessing deep scientific reasoning that cannot be solved via simple retrieval, GPQA \cite{rein2024gpqa} offers a "Google-proof" challenge, with its biology and chemistry subsets posing PhD-level problems. Most recently, HLE \cite{phan2025humanity} has been proposed to address the saturation of existing benchmarks, offering a expert-level test designed to push the frontiers of model performance, with a significant portion dedicated to medicine and biology.

\subsection{Evaluation Methodologies}
Given the diverse array of benchmarks, a critical question arises: how should model performance be effectively assessed against these standards? To address this, current research typically employs three primary evaluation paradigms: human-based evaluation, LLM-based evaluation, and rule-based evaluation.

\noindent \textbf{Human-Based Evaluation.}
Considered the gold standard for assessing clinical utility and safety, human evaluation involves expert clinicians reviewing model outputs against multi-dimensional criteria such as scientific consensus, reasoning correctness, and potential for harm \cite{awasthi2025human, zheng2025large, esmaeilzadeh2025ethical}. Med-PALM \cite{singhal2023large} and Med-PALM 2 \cite{singhal2025toward} pioneered rigorous human evaluation frameworks, employing panels of clinicians to rate long-form answers on axes of accuracy and safety. Similarly, Med-Gemini \cite{saab2024capabilities} utilized expert evaluation to assess performance on long-context tasks. Taking this a step further, AMIE \cite{tu2025towards, mcduff2025towards} utilized a randomized, double-blind study with simulated patients and specialist physicians to evaluate diagnostic dialogue in a realistic, interactive setting. Most recently, PHA \cite{heydari2025anatomy} expanded the scope of human evaluation to a comprehensive multi-stakeholder paradigm, incorporating both end-users and a diverse panel of experts (physicians, data scientists, health coaches). This approach validates over 7,000 interactions to ensure the system is not only medically accurate but also user-aligned and technically robust. Collectively, these evolving frameworks confirm that human evaluation remains the irreplaceable gold standard for verifying clinical safety and utility. However, its high resource intensity constitutes a fundamental bottleneck for scalable model iteration \cite{chang2024survey}.

\noindent \textbf{LLM-Based Evaluation.}
To address the scalability bottlenecks of human review, researchers increasingly employ powerful LLMs (e.g., GPT-4) as surrogate judges to evaluate the outputs of other models. This "LLM-as-a-Judge" paradigm aims to approximate human preference at a fraction of the cost. 
Research initiatives like HuatuoGPT-o1 \cite{chen2412huatuogpt} and Lingshu \cite{xu2025lingshu} have effectively demonstrated the feasibility of utilizing LLMs to assess open-ended medical QA and clinical reasoning quality. 
To further enhance the reliability and granularity of automated scoring, subsequent benchmarks have introduced more sophisticated protocols: HealthBench \cite{arora2025healthbench} utilizes detailed, clinician-curated rubrics to guide the judge model; PHA \cite{heydari2025anatomy} advances this by employing a ``Human-Calibrated'' paradigm, where the LLM ``Autorater'' is explicitly fine-tuned on human expert annotations to maximize alignment with clinical consensus; and MedR-Bench \cite{qiu2025quantifying} deploys an agentic \textit{Reasoning Evaluator} that decomposes reasoning into distinct steps and cross-references them with web-scale resources for verification. 

Nevertheless, as these approaches ultimately depend on the judge model's underlying capabilities, they may still face potential challenges regarding the propagation of biases or the detection of subtle medical hallucinations, suggesting a need for continued vigilance in high-stakes assessments \cite{zheng2023judging, szymanski2025limitations, krumdick2025no}.

\noindent \textbf{Rule-Based Evaluation.}
The most prevalent evaluation method relies on automated metrics tailored to specific task formats: accuracy serves as the standard for multiple-choice benchmarks like MedQA and MMLU, while n-gram overlap scores (e.g., BLEU \cite{papineni2002bleu}, ROUGE \cite{lin2004rouge}) are commonly employed for open-ended generation and question answering tasks \cite{kweon2024ehrnoteqa}. The primary advantage of this paradigm is its objectivity, low cost, and high reproducibility, allowing for consistent comparisons across different models and research groups \cite{chang2024survey}. While these metrics primarily assess the correctness of the final outcome rather than the full granularity of the reasoning process, they remain the essential standard for quantitative benchmarking, providing a reliable signal of a model's domain competency.





\begin{table}[htbp]
    \centering
    \caption{Model performance on existing benchmarks. Background colors denote base LLM families, with each medical LLM inheriting the background color of its corresponding base model. \textbf{Bold} indicates the best overall score; \protect\underline{underlining} marks the best medical LLM within each base model group.}
    \label{tab:model_performance}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccccc}
        \toprule
        \textbf{Model} & \textbf{MedQA} & \textbf{MedMCQA} & \textbf{PubMedQA} & \textbf{GPQA} & \textbf{JMED} & \textbf{ReDis-QA} & \textbf{MedXpertQA} & \textbf{MMLU-Pro} & \textbf{Average} & \textbf{R. I. (\%)} \\
        \midrule
        \multicolumn{11}{c}{\textit{Open-source General LLMs (Base Models)}} \\
        \midrule
        \rowcolor{LightBlue!30} gemma3-4B-it & 0.462 & 0.464 & 0.708 & 0.423 & 0.353 & 0.501 & 0.114 & 0.496 & 0.440 & - \\
        Qwen3-4B-Thinking-2507 & 0.736 & 0.642 & 0.763 & 0.610 & 0.572 & 0.727 & 0.177 & 0.772 & 0.625 & - \\
        \rowcolor{LightYellow} Qwen-2.5-7B-Instruct & 0.582 & 0.562 & 0.748 & 0.474 & 0.580 & 0.667 & 0.131 & 0.623 & 0.546 & - \\
        \rowcolor{Lavender} Meta-Llama-3-8B-Instruct & 0.530 & 0.543 & 0.773 & 0.433 & 0.422 & 0.732 & 0.122 & 0.550 & 0.513 & - \\
        \rowcolor{LightGray!30} Llama-3.1-8B-Instruct & 0.518 & 0.554 & 0.776 & 0.438 & 0.425 & 0.735 & 0.129 & 0.542 & 0.515 & - \\
        Qwen3-8B & \textbf{0.781} & 0.665 & 0.764 & \textbf{0.659} & \textbf{0.668} & 0.778 & 0.182 & \textbf{0.784} & \textbf{0.660} & - \\
        \midrule
        \multicolumn{11}{c}{\textit{Open-source Medical LLMs (vs. Base General LLM)}} \\
        \midrule
        % -------------------------- 基座: gemma3-4B-it (LightBlue) Avg: 0.440 --------------------------
        \rowcolor{LightBlue!30} Medgemma 4B & \protect\underline{0.597} & \protect\underline{0.546} & \protect\underline{0.754} & \protect\underline{0.436} & \protect\underline{0.417} & \protect\underline{0.680} & \protect\underline{0.147} & \protect\underline{0.552} & \protect\underline{0.516} & \protect\underline{\textcolor{ForestGreen}{+17.27}} \\
        % -------------------------- 基座: Qwen-2.5-7B-Instruct (LightYellow) Avg: 0.546 --------------------------
        \rowcolor{LightYellow} ClinicalGPT-R1-Qwen-7B $^{\tnote{\bf a}}$ & 0.431 & 0.526 & 0.670 & 0.462 & 0.078 & 0.649 & 0.112 & 0.559 & 0.436 & \textcolor{red}{-20.15} \\
        \rowcolor{LightYellow} HuatuoGPT-o1-7B & 0.664 & 0.643 & \protect\underline{0.788} & \protect\underline{0.479} & \protect\underline{0.565} & 0.710 & 0.150 & 0.670 & 0.584 & \textcolor{ForestGreen}{+6.92}\\
        % m1-7B Avg calc: (0.719+0.644+0.741+0.479+0.500+0.793+0.201+0.708)/8 = 4.785/8 = 0.598
        \rowcolor{LightYellow} m1-7B-23K & \protect\underline{0.719} & \protect\underline{0.644} & 0.741 & \protect\underline{0.479} & 0.500 & \protect\underline{0.793} & \protect\underline{0.201} & \protect\underline{0.708} & \protect\underline{0.598} & \protect\underline{\textcolor{ForestGreen}{+9.57}} \\
        % -------------------------- 基座: Meta-Llama-3-8B-Instruct (Lavender) Avg: 0.513 --------------------------
        % Med42 Avg: 4.322/8 = 0.540
        \rowcolor{Lavender} Med42-v2-8B & 0.562 & 0.582 & \protect\underline{0.782} & 0.456 & 0.424 & \protect\underline{\textbf{0.839}} & 0.136 & 0.541 & 0.540 & \textcolor{ForestGreen}{+5.29} \\
        % Meerkat Avg: 4.428/8 = 0.5535 -> 0.554
        \rowcolor{Lavender} Meerkat-8B & \protect\underline{0.661} & \protect\underline{0.587} & 0.764 & \protect\underline{0.474} & \protect\underline{0.431} & 0.787 & \protect\underline{0.148} & \protect\underline{0.576} & \protect\underline{0.554} & \protect\underline{\textcolor{ForestGreen}{+7.87}} \\
        % -------------------------- 基座: Llama-3.1-8B-Instruct (LightGray) Avg: 0.515 --------------------------
        % Adathink Avg: 4.289/8 = 0.536
        \rowcolor{LightGray!30} Adathink-Med-Llama-8B & 0.581 & 0.572 & 0.780 & 0.433 & 0.399 & 0.778 & 0.162 & 0.584 & 0.536 & \textcolor{ForestGreen}{+4.18} \\
        % AlphaMed Avg: 4.723/8 = 0.590
        \rowcolor{LightGray!30} AlphaMed-8B & 0.705 & 0.649 & 0.785 & \protect\underline{0.564} & 0.294 & 0.833 & \protect\underline{\textbf{0.230}} & 0.663 & 0.590 & \textcolor{ForestGreen}{+14.72} \\
        % BioMed Avg: 4.900/8 = 0.6125 -> 0.613
        \rowcolor{LightGray!30} BioMed-R1-8B & \protect\underline{0.769} & \protect\underline{\textbf{0.667}} & 0.783 & 0.556 & 0.404 & 0.835 & 0.204 & \protect\underline{0.682} & \protect\underline{0.613} & \protect\underline{\textcolor{ForestGreen}{+19.02}} \\
        % Huatuo-o1-8B Avg: 4.627/8 = 0.578
        \rowcolor{LightGray!30} HuatuoGPT-o1-8B & 0.723 & 0.643 & 0.788 & 0.536 & 0.352 & 0.793 & 0.164 & 0.628 & 0.578 & \textcolor{ForestGreen}{+12.39} \\
        % UltraMedical Avg: 4.629/8 = 0.5786 -> 0.579
        \rowcolor{LightGray!30} Llama-3.1-8B-UltraMedical & 0.698 & 0.622 & \protect\underline{\textbf{0.789}} & 0.462 & \protect\underline{0.447} & 0.815 & 0.162 & 0.634 & 0.579 & \textcolor{ForestGreen}{+12.44} \\
        % MedReason Avg: 4.427/8 = 0.553
        \rowcolor{LightGray!30} MedReason-8B & 0.653 & 0.605 & 0.733 & 0.487 & 0.355 & 0.754 & 0.218 & 0.622 & 0.553 & \textcolor{ForestGreen}{+7.53} \\
        % MedS3 Avg: 4.682/8 = 0.585
        \rowcolor{LightGray!30} MedS$^3$-8B & 0.684 & 0.639 & 0.781 & 0.495 & 0.414 & \protect\underline{\textbf{0.839}} & 0.171 & 0.659 & 0.585 & \textcolor{ForestGreen}{+13.72} \\
        \bottomrule
    \end{tabular}%
    }
\begin{tablenotes}
\item \textit{Abbreviations}: R.I.: Relative Improvement (compared to the corresponding base general LLM).

\end{tablenotes} 
\end{table}

\subsection{Comprehensive Evaluation of Model Performance}
Despite the availability of numerous datasets, the field of medical reasoning LLMs lacks a unified benchmarking standard, with different studies often selecting disparate sets of benchmarks for assessment. While datasets such as MedQA, PubMedQA, and MedMCQA are widely adopted, concerns persist regarding potential data leakage and the risk of models overfitting to these specific test sets \cite{singhal2023large, nori2023capabilities}. Furthermore, even when utilizing objective, rule-based evaluation metrics, reported performance for identical models on the same benchmarks can vary. These discrepancies are primarily attributable to differences in prompt engineering and the specific rules employed for answer parsing. To address these disparities and provide a holistic view of performance, we conducted a comprehensive evaluation from two complementary perspectives: examining distinct medical reasoning models and assessing various enhancement methodologies across a diverse suite of benchmarks. Specifically, we selected MedQA (5-options), PubMedQA, and MedMCQA as standard benchmarks, complemented by the medical subsets of MMLU-Pro and GPQA. Furthermore, ReDis-QA was included to assess generalization to rare diseases, MedXpertQA to test expert-level reasoning, and JMED to evaluate clinical reasoning capabilities within the Chinese context.


To validate the effectiveness of existing training approaches tailored for enhancing medical reasoning in LLMs, we evaluated selected open-source medical LLMs against their respective general base models across the chosen benchmarks, with the comprehensive results presented in Table~\ref{tab:model_performance}. We quantified the efficacy of domain adaptation by calculating the relative improvement of each medical model over its general counterpart. Considering computational constraints and the need for equitable horizontal comparison, we restricted our evaluation to open-source models with parameter sizes under 10B. Furthermore, while we observed that the majority of contemporary research is built upon Qwen-2.5-7B-Instruct and Llama-3.1-8B-Instruct, we additionally incorporated the emerging Qwen3-4B-Thinking-2507 and Qwen3-8B \cite{yang2025qwen3technicalreport} to assess the performance of the new generation general LLMs on medical benchmarks. Detailed experimental settings are provided in Appendix \ref{Appendix 1}.


The results indicate that domain-specific adaptation consistently enhances reasoning capabilities, with models such as Medgemma 4B and BioMed-R1-8B achieving relative improvements of approximately 17\% and 20\% over their base counterparts, barring ClinicalGPT-R1 where performance regression appears linked to weight anomalies (see Appendix \ref{Appendix B}). Performance nuances exist across tasks: on the real-world Chinese benchmark JMED, most models struggle likely due to English-centric training, whereas Qwen-based variants (e.g., HuatuoGPT-o1, m1) leverage their linguistic foundation to perform well, and AlphaMed-8B's leading score on the highly difficult MedXpertQA suggests the specific utility of reinforcement learning for complex problem solving. Significantly, the frontier of general capabilities is advancing rapidly; the untuned Qwen3-8B achieves the highest overall average, and even the smaller Qwen3-4B-Thinking outperforms many larger specialized models, highlighting a critical imperative to update current training pipelines.

% \begin{table}[htbp]
% \centering
% % 将表格宽度调整为文本宽度
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% Model & MedQA & MedMCQA & PubMedQA & GPQA & JMED & ReDis-QA & MedXpertQA & MMLU-Pro & Average & R. I. (\%) \\
% \midrule
% Llama-3.1-8B-Instruct & 0.518 & 0.554 & 0.776 & 0.438 & 0.425 & 0.735 & 0.129 & 0.542 & 0.515 & - \\
% +SC (n=5) & 0.322 & 0.394 & 0.781 & 0.379 & 0.163 & 0.477 & 0.121 & 0.417 & 0.381 & \\
% +ER (n=5) & 0.563 & 0.552 & 0.774 & 0.479 & 0.421 & 0.762 & 0.126 & 0.567 & 0.531 & \\
% +Medprompt & & & & & & & & & & \\
% +MedAgents & & & & & & & & & & \\
% \midrule
% Qwen-2.5-7B-Instruct & 0.582 & 0.562 & 0.748 & 0.474 & 0.580 & 0.667 & 0.131 & 0.623 & 0.546 & - \\
% +SC (n=5) & & & & & & & & & & \textcolor{ForestGreen}{+1.11}\\
% +ER (n=5) & 0.588 & 0.572 & 0.769 & 0.505 & 0.597 & 0.690 & 0.129 & 0.639 & 0.561 & \\
% +Medprompt & 0.603 & 0.487 & 0.638 & 0.523 & 0.581 & 0.523 & 0.122 & 0.648 & 0.515 & \\
% +MedAgents & & & & & & & & & & \\
% \midrule
% HuatuoGPT-o1-8B & 0.723 & 0.643 & 0.788 & 0.536 & 0.342 & 0.793 & 0.164 & 0.628 & 0.577 & - \\
% +SC (n=5) & 0.715 & 0.640 & 0.799 & 0.538 & 0.3 & 0.813 & 0.171 & 0.641 & 0.577 & \\
% +ER (n=5) & & & & & & & & & & \\
% +Medprompt & & & & & & & & & & \\
% +MedAgents & & & & & & & & & & \\
% \midrule
% Llama-3.1-8B-UltraMedical & 0.698 & 0.622 & 0.789 & 0.462 & 0.347 & 0.815 & 0.162 & 0.634 & 0.566 & - \\
% +SC (n=5) & & & & & & & & & & \\
% +ER (n=5) & 0.720 &  & & & & & & & & \\
% +Medprompt & & & & & & & & & & \\
% +MedAgents & & & & & & & & & & \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Impact of various training-free strategies on model performance.}
% \end{table}
